Improving Augmentation and Evaluation Schemes for Semantic Image Synthesis

Despite data augmentation being a de facto technique for boosting the performance of deep neural networks, little attention has been paid to developing augmentation strategies for generative adversarial networks (GANs). To this end, we introduce a novel augmentation scheme designed specifically for GAN-based semantic image synthesis models. We propose to randomly warp object shapes in the semantic label maps used as an input to the generator. The local shape discrepancies between the warped and non-warped label maps and images enable the GAN to learn better the structural and geometric details of the scene and thus to improve the quality of generated images. While benchmarking the augmented GAN models against their vanilla counterparts, we discover that the quantification metrics reported in the previous semantic image synthesis studies are strongly biased towards specific semantic classes as they are derived via an external pre-trained segmentation network. We therefore propose to improve the established semantic image synthesis evaluation scheme by analyzing separately the performance of generated images on the biased and unbiased classes for the given segmentation network. Finally, we show strong quantitative and qualitative improvements obtained with our augmentation scheme, on both class splits, using state-of-the-art semantic image synthesis models across three different datasets. On average across COCO-Stuff, ADE20K and Cityscapes datasets, the augmented models outperform their vanilla counterparts by ~3 mIoU and ~10 FID points.

==> figures/ade20k_qualitative.tex <==


\begin{figure}[H]
	\centering
	\setlength{\tabcolsep}{0em}
	\renewcommand{\arraystretch}{0}
	
	\vspace{-1em}
	\hfill{}%
	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
		
		\centering
		
		Label map & Real image & Pix2PixHD & Pix2PixHD-el & Pix2PixHD-aug \vspace{0.05cm} \tabularnewline
		
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/gt/ADE_val_00000033.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/org_img/ADE_val_00000033.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/baseline/ADE_val_00000033.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/baseline_el/ADE_val_00000033.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/augmented/ADE_val_00000033.png} \vspace{0.05cm} \tabularnewline
		
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/gt/ADE_val_00000088.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/org_img/ADE_val_00000088.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/baseline/ADE_val_00000088.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/baseline_el/ADE_val_00000088.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/augmented/ADE_val_00000088.png} \vspace{0.05cm} \tabularnewline
		
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/gt/ADE_val_00000258.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/org_img/ADE_val_00000258.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/baseline/ADE_val_00000258.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/baseline_el/ADE_val_00000258.png} & {\footnotesize{}}
		\includegraphics[width=0.19\linewidth]{figures/models/pix2pixhd/ade20k/augmented/ADE_val_00000258.png} 
		
	\end{tabular}
	\caption{Semantic image synthesis results on ADE20K using Pix2PixHD baselines and the augmented model. Best viewed in color.}
	\vspace{-1em}
	\label{fig:ade20k_qualitative}
\end{figure}

==> figures/cityscapes_qualitative.tex <==


\begin{figure}[H]
	\centering
	\setlength{\tabcolsep}{0em}
	\renewcommand{\arraystretch}{0}
	
	\vspace{-1em}
	\hfill{}%
	\begin{tabular}{@{}c@{}c@{}c@{}}
		
		\centering
		
		CC-FPSE & CC-FPSE-el & CC-FPSE-aug \vspace{0.05cm} \tabularnewline
		
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/baseline/munster_000100_000019_leftImg8bit.png} & {\footnotesize{}}
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/baseline_el/munster_000100_000019_leftImg8bit.png} & {\footnotesize{}}
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/augmented/munster_000100_000019_leftImg8bit.png} \vspace{0.05cm} \tabularnewline
		
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/baseline/munster_000141_000019_leftImg8bit.png} & {\footnotesize{}}
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/baseline_el/munster_000141_000019_leftImg8bit.png} & {\footnotesize{}}
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/augmented/munster_000141_000019_leftImg8bit.png} \vspace{0.05cm} \tabularnewline 
		
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/baseline/munster_000139_000019_leftImg8bit.png} & {\footnotesize{}}
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/baseline_el/munster_000139_000019_leftImg8bit.png} & {\footnotesize{}}
		\includegraphics[width=0.32\linewidth]{figures/models/ccfpse/cityscapes/augmented/munster_000139_000019_leftImg8bit.png} \vspace{0.05cm} 
		
	\end{tabular}
	\caption{Semantic image synthesis results on Cityscapes using CC-FPSE baselines and the augmented model. For a better comparison, the label map and the real images are moved to the supplementary data. Best viewed in color.}
	\vspace{-1em}
	\label{fig:cityscapes_qualitative}
\end{figure}

==> figures/warping_examples.tex <==


\begin{wrapfigure}{l}{0.4\textwidth}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/warping_examples/warping_examples.pdf}
	\vspace{-1.5em}
	\caption{Original and warped label maps and the corresponding images. The key-points sampled using the edge maps are shown in the original images in the second column. The warped images in the last column are shown only for the ease of illustration.}
	\label{fig:warping_examples}
\end{wrapfigure}

==> sections/acknowledgements.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.

Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> sections/broader_impact.tex <==
\section*{Broader Impact}

The potential broader impact of this submission may fall into several different areas. Our work improves the fidelity of images synthesized using the existing generative adversarial network-based semantic image synthesis (SIS) models as well as proposes a fair evaluation scheme for future SIS methods. 

Images generated with our proposed augmentation strategy can be utilized as alternatives for the cases where collecting real data is either prohibitive or very challenging. This includes the situations in which privacy-sensitive data cannot be used without the consent of a legitimate owner, such as images with people or scenes containing confidential information. In such scenarios, the data generated by SIS models may potentially serve as replacement and preserve the privacy of people. Our proposed approach can also be used to generate diversified synthetic images for enlarging the training sets in applications that are highly data-driven, such as autonomous driving. In the same vein, the synthetic images can be used to mitigate the intrinsic biases present in the original training datasets and to improve the generalization of the trained models. For example, by artificially adding instances of rare categories in the training images. 

As the methods for conditional image generation are getting better, the risk of their misuse for image or video tampering is also increasing. One potential application where the proposed augmentation technique can be abused is the generation of deepfakes. SIS models allow to easily manipulate objects in the synthesized images by directly modifying the semantic segments in the input label map. The images generated using the augmented SIS models are of higher fidelity than the samples from the respective baselines, and thus are harder to identify as fake for an independent human observer.

A second contribution of this work is the extended evaluation benchmark for SIS. By proposing to split the semantic segmentation metrics in two groups, for biased and unbiased classes, we can fairly analyze the semantic classes on which SIS models improve most. 
%This allows to stratify novel SIS approaches that equitably improve over the unbiased semantic classes, which are usually under-represented in the training set, and thus are more challenging to synthesize. 
This allows to distinguish novel SIS approaches that equitably improve over both, the biased and unbiased semantic classes, where the latter are usually under-represented in the training set, and thus are more challenging to synthesize. The proposed extended evaluation helps to promote fairness in benchmarking SIS models, as it weakens the adverse effects of potential biases present in the collected data.

Overall, the contributions made in this work can be seen as a step forward towards privacy-preserving and fair AI.



